Kepler-1656b: a Dense Sub-Saturn With an Extreme Eccentricity

Kepler-1656b is a 5 $R_E$ planet with an orbital period of 32 days initially detected by the prime Kepler mission. We obtained precision radial velocities of Kepler-1656 with Keck/HIRES in order to confirm the planet and to characterize its mass and orbital eccentricity. With a mass of $48 \pm 4 M_E$, Kepler-1656b is more massive than most planets of comparable size. Its high mass implies that a significant fraction, roughly 80%, of the planet's total mass is in high density material such as rock/iron, with the remaining mass in a low density H/He envelope. The planet also has a high eccentricity of $0.84 \pm 0.01$, the largest measured eccentricity for any planet less than 100 $M_E$. The planet's high density and high eccentricity may be the result of one or more scattering and merger events during or after the dispersal of the protoplanetary disk.

==> tab_rv.tex <==
% time, mnvel, errvel, S-value
2457521.024708 &   11.147078 &   1.979005 &   0.164600 \\
2457556.928676 &   0.349223 &   2.128298 &   0.160900 \\
2457556.960864 &   3.059876 &   2.745865 &   0.167800 \\
2457562.055606 &   10.944738 &   1.941770 &   0.158400 \\
2457562.924973 &   6.599705 &   1.773373 &   0.158000 \\
2457571.036004 &   2.433189 &   2.570893 &   0.124000 \\
2457581.987078 &   -6.131009 &   1.900433 &   0.161500 \\
2457582.025562 &   0.759614 &   1.659714 &   0.157200 \\
2457582.124949 &   5.088809 &   1.849964 &   0.157000 \\
2457582.981513 &   0.884146 &   2.011170 &   0.156500 \\
2457583.890265 &   1.334622 &   1.843640 &   0.156500 \\
2457584.844768 &   -4.473089 &   1.891837 &   0.155400 \\
2457585.869641 &   0.790008 &   1.871684 &   0.158500 \\
2457586.889340 &   2.061245 &   1.839356 &   0.157300 \\
2457587.891376 &   2.546408 &   1.983551 &   0.157700 \\
2457592.006120 &   3.715565 &   1.981217 &   0.157100 \\
2457592.068215 &   3.853674 &   2.224780 &   0.151700 \\
2457592.117092 &   -0.660168 &   2.516992 &   0.139900 \\
2457596.028317 &   2.767621 &   2.398304 &   0.138700 \\
2457596.935289 &   10.119999 &   2.228440 &   0.150200 \\
2457598.946393 &   23.427343 &   1.908320 &   0.151700 \\
2457599.995456 &   -2.881136 &   2.012203 &   0.156100 \\
2457600.936013 &   -12.150145 &   2.063175 &   0.149400 \\
2457618.871649 &   -0.694156 &   2.011001 &   0.150300 \\
2457620.934583 &   1.984183 &   2.488059 &   0.152900 \\
2457651.830117 &   3.141548 &   1.893627 &   0.144000 \\
2457651.894894 &   -0.976624 &   1.726820 &   0.148500 \\
2457651.937404 &   2.340268 &   1.895439 &   0.145000 \\
2457652.826904 &   -3.053816 &   1.933326 &   0.148100 \\
2457652.877145 &   -2.637414 &   2.152421 &   0.143400 \\
2457652.915835 &   5.327667 &   1.936317 &   0.144800 \\
2457653.861397 &   -3.935982 &   2.109695 &   0.145300 \\
2457668.786163 &   -8.801960 &   1.831618 &   0.150500 \\
2457668.832365 &   -12.269308 &   1.887944 &   0.150300 \\
2457668.884365 &   -2.118365 &   2.055461 &   0.147000 \\
2457671.728041 &   -12.212072 &   2.105411 &   0.147600 \\
2457671.799670 &   -7.752098 &   1.898558 &   0.147600 \\
2457672.729766 &   -8.344154 &   2.030991 &   0.146600 \\
2457672.793849 &   -4.942202 &   1.929036 &   0.148600 \\
2457672.859957 &   -10.869319 &   2.121530 &   0.144200 \\
2457678.721050 &   -0.338171 &   2.031386 &   0.144800 \\
2457678.768906 &   0.909627 &   2.090707 &   0.138100 \\
2457678.837919 &   -7.108448 &   2.470486 &   0.123500 \\
2457679.716015 &   -3.034282 &   1.814404 &   0.143300 \\
2457679.815328 &   -2.883801 &   2.743264 &   0.142700 \\
2457697.710100 &   -17.352768 &   2.110918 &   0.147300 \\
2457697.739415 &   -9.683211 &   2.013195 &   0.145300 \\
2457697.782249 &   -3.798056 &   1.894789 &   0.137200 \\
2457703.764132 &   -5.593917 &   2.059458 &   0.149300 \\
2457703.784062 &   -1.455062 &   2.187479 &   0.148800 \\
2457703.793887 &   -1.691778 &   2.159871 &   0.154000 \\
2457711.691181 &   -3.049811 &   2.124023 &   0.144500 \\
2457712.693063 &   0.464530 &   2.786950 &   0.133200 \\
2457714.720104 &   -6.062359 &   2.267531 &   0.144000 \\
2457718.706080 &   2.282086 &   2.096136 &   0.138300 \\
2457795.161993 &   -5.293156 &   2.086357 &   0.144000 \\
2457829.100800 &   -4.049408 &   2.046983 &   0.157700 \\
2457829.117005 &   2.015369 &   1.995722 &   0.160300 \\
2457829.141902 &   0.262205 &   1.909305 &   0.159400 \\
2457831.088544 &   -0.475611 &   2.145882 &   0.157900 \\
2457831.116531 &   -4.508786 &   1.941528 &   0.159000 \\
2457831.142655 &   -5.191402 &   1.885407 &   0.156100 \\
2457853.082413 &   -10.324095 &   2.379127 &   0.135800 \\
2457853.129915 &   -6.719064 &   2.462444 &   0.124100 \\
2457854.075943 &   -1.226229 &   1.891020 &   0.155300 \\
2457855.092251 &   -8.700387 &   2.004681 &   0.152000 \\
2457855.134915 &   -7.715930 &   2.062163 &   0.154200 \\
2457887.049010 &   -12.162772 &   1.976625 &   0.159800 \\
2457887.099707 &   -9.569731 &   1.828375 &   0.161200 \\
2457888.060428 &   -1.816287 &   1.934826 &   0.159400 \\
2457888.084503 &   -6.346849 &   1.795838 &   0.155300 \\
2457888.119181 &   -12.598350 &   2.096337 &   0.156100 \\
2457911.922610 &   1.781379 &   2.023644 &   0.151800 \\
2457911.960748 &   7.673350 &   1.877174 &   0.153300 \\
2457912.007289 &   5.979197 &   1.902790 &   0.153400 \\
2457912.969121 &   15.105227 &   1.901519 &   0.153200 \\
2457913.019990 &   11.503537 &   1.982063 &   0.152500 \\
2457925.016616 &   -1.263918 &   2.255611 &   0.153200 \\
2457925.052346 &   -7.448377 &   2.167172 &   0.131300 \\
2457926.026114 &   -7.682335 &   1.982993 &   0.153500 \\
2457926.062782 &   -1.261804 &   2.051849 &   0.153600 \\
2457927.002834 &   -2.071524 &   1.915379 &   0.155700 \\
2457927.037302 &   2.389149 &   2.076244 &   0.153000 \\
2457927.059617 &   -7.953885 &   1.978552 &   0.155200 \\
2457932.974434 &   -3.217500 &   1.943892 &   0.152400 \\
2457933.001958 &   2.048273 &   1.878062 &   0.153900 \\
2457933.924644 &   0.339758 &   1.903917 &   0.147900 \\
2457933.970292 &   -2.312984 &   1.720528 &   0.153500 \\
2457934.005941 &   2.160233 &   1.817799 &   0.152400 \\
2457934.854007 &   3.277567 &   1.977793 &   0.152700 \\
2457934.887411 &   -0.554634 &   1.918180 &   0.152400 \\
2457934.937874 &   -3.288830 &   1.969868 &   0.154800 \\
2457939.928088 &   7.257094 &   2.119608 &   0.143900 \\
2457940.944486 &   7.034995 &   1.889999 &   0.149700 \\
2457942.953435 &   16.082314 &   2.006530 &   0.152700 \\
2457943.007891 &   2.457911 &   1.997617 &   0.145800 \\
2457944.954742 &   19.429260 &   1.917948 &   0.155200 \\
2457945.003562 &   13.902115 &   2.236573 &   0.141500 \\
2457945.993208 &   18.233268 &   2.032434 &   0.140200 \\
2457946.041298 &   22.465483 &   2.057946 &   0.197100 \\

==> tab_subsaturns-1gyr.tex <==
% name radius mass density ecc teq cmf notes
Kepler-4 b & 1 & 4.00^{ +0.21 }_{ -0.21 } & 24.5^{ +3.8 }_{ -3.8 } & 2.09^{ +0.53 }_{ -0.44 } & \nodata  & 1597 & 94.2^{ +1.3 }_{ -1.2 } & 0.17 & \cite{Borucki10}\\
GJ 436 b & 1 & 4.17^{ +0.17 }_{ -0.17 } & 22.1^{ +2.3 }_{ -2.3 } & 1.67^{ +0.30 }_{ -0.26 } & 0.1383^{ +0.0002 }_{ -0.0002 } & 659 & 89.1^{ +1.6 }_{ -1.7 } & \nodata  & \cite{Butler04}\\
Kepler-11 e & 6 & 4.19^{ +0.07 }_{ -0.09 } & 8.0^{ +1.5 }_{ -2.1 } & 0.60^{ +0.15 }_{ -0.14 } & 0.0120^{ +0.0060 }_{ -0.0060 } & 630 & 87.6^{ +0.8 }_{ -0.7 } & -0.04 & \cite{Lissauer13}\\
Kepler-413 b & 1 & 4.35^{ +0.10 }_{ -0.10 } & 51.0^{ +22.0 }_{ -21.0 } & 2.40^{ +1.00 }_{ -1.00 } & 0.1185^{ +0.0018 }_{ -0.0017 } & 348 & 90.4^{ +1.5 }_{ -2.9 } & \nodata  & \cite{Kostov14}\\
K2-27 b & 1 & 4.48^{ +0.23 }_{ -0.23 } & 30.9^{ +4.6 }_{ -4.6 } & 1.88^{ +0.46 }_{ -0.38 } & 0.2510^{ +0.0880 }_{ -0.0880 } & 910 & 87.9^{ +2.5 }_{ -2.4 } & 0.13 & \cite{petigura17}k\\
Kepler-223 e & 4 & 4.60^{ +0.27 }_{ -0.41 } & 4.8^{ +1.4 }_{ -1.2 } & 0.27^{ +0.11 }_{ -0.09 } & 0.0510^{ +0.0190 }_{ -0.0190 } & 944 & 87.2^{ +2.9 }_{ -2.3 } & 0.06 & \cite{Mills16}\\
HAT-P-11 b & 1 & 4.73^{ +0.16 }_{ -0.16 } & 25.7^{ +2.9 }_{ -2.9 } & 1.34^{ +0.22 }_{ -0.20 } & 0.1980^{ +0.0460 }_{ -0.0460 } & 861 & 84.8^{ +1.5 }_{ -1.4 } & 0.31 & \cite{Bakos10}\\
K2-32 b & 3 & 5.13^{ +0.28 }_{ -0.28 } & 16.5^{ +2.7 }_{ -2.7 } & 0.67^{ +0.18 }_{ -0.15 } & \nodata  & 815 & 80.9^{ +2.3 }_{ -2.9 } & -0.02 & \cite{petigura17}\\
Kepler-25 c & 3 & 5.20^{ +0.09 }_{ -0.09 } & 24.6^{ +5.7 }_{ -5.7 } & 0.96^{ +0.24 }_{ -0.23 } & \nodata  & 1018 & 81.4^{ +0.7 }_{ -0.7 } & -0.04 & \cite{Marcy14}\\
Kepler-223 d & 4 & 5.24^{ +0.26 }_{ -0.45 } & 8.0^{ +1.5 }_{ -1.3 } & 0.30^{ +0.10 }_{ -0.07 } & 0.0370^{ +0.0180 }_{ -0.0170 } & 1040 & 82.1^{ +2.5 }_{ -2.3 } & 0.06 & \cite{Mills16}\\
EPIC-2117 b & 1 & 5.37^{ +0.44 }_{ -0.44 } & 68.8^{ +7.7 }_{ -7.7 } & 2.43^{ +0.80 }_{ -0.57 } & 0.2560^{ +0.0760 }_{ -0.1000 } & 1440 & 85.5^{ +4.2 }_{ -3.8 } & 0.33 & \cite{petigura17}\\
Kepler-18 c & 3 & 5.49^{ +0.26 }_{ -0.26 } & 17.3^{ +1.9 }_{ -1.9 } & 0.57^{ +0.12 }_{ -0.10 } & \nodata  & 979 & 78.3^{ +2.4 }_{ -2.5 } & 0.19 & \cite{Cochran11}\\
K2-24 b & 2 & 5.68^{ +0.56 }_{ -0.56 } & 21.0^{ +5.4 }_{ -5.4 } & 0.62^{ +0.31 }_{ -0.22 } & \nodata  & 766 & 75.3^{ +5.8 }_{ -5.0 } & 0.42 & \cite{Petigura16}\\
K2-39 b & 1 & 5.71^{ +0.63 }_{ -0.63 } & 39.7^{ +4.6 }_{ -4.6 } & 1.16^{ +0.54 }_{ -0.34 } & 0.1500^{ +0.0760 }_{ -0.0760 } & 1689 & 84.2^{ +4.5 }_{ -4.1 } & 0.43 & \cite{petigura17}\\
Kepler-101 b & 2 & 5.77^{ +0.85 }_{ -0.79 } & 51.1^{ +5.1 }_{ -4.7 } & 1.46^{ +0.90 }_{ -0.50 } & 0.0860^{ +0.0800 }_{ -0.0590 } & 1547 & 82.6^{ +6.6 }_{ -6.8 } & 0.33 & \cite{Bonomo14}\\
Kepler-87 c & 2 & 6.14^{ +0.29 }_{ -0.29 } & 6.4^{ +0.8 }_{ -0.8 } & 0.15^{ +0.03 }_{ -0.03 } & 0.0390^{ +0.0120 }_{ -0.0120 } & 440 & 72.3^{ +2.2 }_{ -2.1 } & -0.17 & \cite{Ofir14}\\
HATS-7 b & 1 & 6.31^{ +0.52 }_{ -0.38 } & 38.1^{ +3.8 }_{ -3.8 } & 0.83^{ +0.23 }_{ -0.17 } & \nodata  & 1070 & 71.3^{ +4.7 }_{ -5.9 } & 0.25 & \cite{Bakos15}\\
HAT-P-26 b & 1 & 6.33^{ +0.81 }_{ -0.36 } & 18.8^{ +2.2 }_{ -2.2 } & 0.40^{ +0.15 }_{ -0.10 } & 0.1240^{ +0.0600 }_{ -0.0600 } & 981 & 70.6^{ +5.2 }_{ -6.7 } & -0.04 & \cite{Hartman11}\\
CoRoT-8 b & 1 & 6.39^{ +0.22 }_{ -0.22 } & 69.9^{ +9.5 }_{ -9.5 } & 1.47^{ +0.27 }_{ -0.25 } & \nodata  & 844 & 71.4^{ +2.3 }_{ -2.5 } & 0.30 & \cite{Borde10}\\
Kepler-56 b & 3 & 6.51^{ +0.29 }_{ -0.28 } & 22.1^{ +3.9 }_{ -3.6 } & 0.44^{ +0.10 }_{ -0.09 } & \nodata  & 1479 & 78.0^{ +2.4 }_{ -2.5 } & 0.37 & \cite{Huber13}\\
Kepler-18 d & 3 & 6.98^{ +0.33 }_{ -0.33 } & 16.4^{ +1.4 }_{ -1.4 } & 0.26^{ +0.05 }_{ -0.04 } & 0.0000^{ + }_{  } & 784 & 62.5^{ +3.4 }_{ -3.6 } & 0.19 & \cite{Cochran11}\\
Kepler-79 d & 4 & 7.16^{ +0.13 }_{ -0.16 } & 6.0^{ +2.1 }_{ -1.6 } & 0.09^{ +0.03 }_{ -0.03 } & 0.0250^{ +0.0590 }_{ -0.0230 } & 626 & 67.3^{ +4.0 }_{ -3.3 } & -0.02 & \cite{Jontof-Hutter14}.\\
K2-24 c & 2 & 7.82^{ +0.72 }_{ -0.72 } & 27.0^{ +6.9 }_{ -6.9 } & 0.31^{ +0.14 }_{ -0.10 } & \nodata  & 605 & 51.5^{ +6.9 }_{ -8.9 } & 0.42 & \cite{Petigura16}\\
KOI-367 b & 1 & 5.03_{ -0.53 }^{+0.53} & 48.5_{ -3.68}^{+3.99} & 2.11_{ -0.56 }^{+0.86} & 0.833_{-0.013}^{+0.013} & 652 & 82.2_{-6.2}^{+5.9} & 0.189 & This work\\

==> tab_subsaturns-2gyr.tex <==
% name radius mass density ecc teq cmf notes
Kepler-4 b & 1 & 4.00^{ +0.21 }_{ -0.21 } & 24.5^{ +3.8 }_{ -3.8 } & 2.09^{ +0.53 }_{ -0.44 } & \nodata  & 1597 & 93.6^{ +1.5 }_{ -1.2 } & 0.17 & \cite{Borucki10}\\
GJ 436 b & 1 & 4.17^{ +0.17 }_{ -0.17 } & 22.1^{ +2.3 }_{ -2.3 } & 1.67^{ +0.30 }_{ -0.26 } & 0.1383^{ +0.0002 }_{ -0.0002 } & 659 & 88.3^{ +1.9 }_{ -1.8 } & \nodata  & \cite{Butler04}. NEA gives no age. Adopted $5\pm2 Gyr$\\
Kepler-11 e & 6 & 4.19^{ +0.07 }_{ -0.09 } & 8.0^{ +1.5 }_{ -2.1 } & 0.60^{ +0.15 }_{ -0.14 } & 0.0120^{ +0.0060 }_{ -0.0060 } & 630 & 86.5^{ +0.8 }_{ -0.8 } & -0.04 & \cite{Lissauer13}\\
Kepler-413 b & 1 & 4.35^{ +0.10 }_{ -0.10 } & 51.0^{ +22.0 }_{ -21.0 } & 2.40^{ +1.00 }_{ -1.00 } & 0.1185^{ +0.0018 }_{ -0.0017 } & 348 & 90.0^{ +1.5 }_{ -3.4 } & \nodata  & \cite{Kostov14}. NEA gives no age. Adopted $5\pm2$~Gyr\\
K2-27 b & 1 & 4.48^{ +0.23 }_{ -0.23 } & 30.9^{ +4.6 }_{ -4.6 } & 1.88^{ +0.46 }_{ -0.38 } & 0.2510^{ +0.0880 }_{ -0.0880 } & 910 & 87.0^{ +2.8 }_{ -2.4 } & 0.13 & \cite{petigura17}\\
Kepler-223 e & 4 & 4.60^{ +0.27 }_{ -0.41 } & 4.8^{ +1.4 }_{ -1.2 } & 0.27^{ +0.11 }_{ -0.09 } & 0.0510^{ +0.0190 }_{ -0.0190 } & 944 & 85.5^{ +2.9 }_{ -2.5 } & 0.06 & \cite{Mills16}\\
HAT-P-11 b & 1 & 4.73^{ +0.16 }_{ -0.16 } & 25.7^{ +2.9 }_{ -2.9 } & 1.34^{ +0.22 }_{ -0.20 } & 0.1980^{ +0.0460 }_{ -0.0460 } & 861 & 83.9^{ +1.5 }_{ -1.4 } & 0.31 & \cite{Bakos10}\\
K2-32 b & 3 & 5.13^{ +0.28 }_{ -0.28 } & 16.5^{ +2.7 }_{ -2.7 } & 0.67^{ +0.18 }_{ -0.15 } & \nodata  & 815 & 79.6^{ +2.4 }_{ -3.4 } & -0.02 & \cite{petigura17}\\
Kepler-25 c & 3 & 5.20^{ +0.09 }_{ -0.09 } & 24.6^{ +5.7 }_{ -5.7 } & 0.96^{ +0.24 }_{ -0.23 } & \nodata  & 1018 & 80.3^{ +0.8 }_{ -1.0 } & -0.04 & \cite{Marcy14}. NEA gives 11 Gyr with no uncertainties. Adopted $11\pm2$ Gyr.\\
Kepler-223 d & 4 & 5.24^{ +0.26 }_{ -0.45 } & 8.0^{ +1.5 }_{ -1.3 } & 0.30^{ +0.10 }_{ -0.07 } & 0.0370^{ +0.0180 }_{ -0.0170 } & 1040 & 80.5^{ +2.6 }_{ -3.2 } & 0.06 & \cite{Mills16}. Did not report age. Adopted $5\pm2 Gyr$\\
EPIC-2117 b & 1 & 5.37^{ +0.44 }_{ -0.44 } & 68.8^{ +7.7 }_{ -7.7 } & 2.43^{ +0.80 }_{ -0.57 } & 0.2560^{ +0.0760 }_{ -0.1000 } & 1440 & 84.7^{ +4.3 }_{ -3.9 } & 0.33 & \cite{petigura17}\\
Kepler-18 c & 3 & 5.49^{ +0.26 }_{ -0.26 } & 17.3^{ +1.9 }_{ -1.9 } & 0.57^{ +0.12 }_{ -0.10 } & \nodata  & 979 & 76.4^{ +2.8 }_{ -2.6 } & 0.19 & \cite{Cochran11}\\
K2-24 b & 2 & 5.68^{ +0.56 }_{ -0.56 } & 21.0^{ +5.4 }_{ -5.4 } & 0.62^{ +0.31 }_{ -0.22 } & \nodata  & 766 & 73.5^{ +6.6 }_{ -6.2 } & 0.42 & \cite{Petigura16}\\
K2-39 b & 1 & 5.71^{ +0.63 }_{ -0.63 } & 39.7^{ +4.6 }_{ -4.6 } & 1.16^{ +0.54 }_{ -0.34 } & 0.1500^{ +0.0760 }_{ -0.0760 } & 1689 & 83.0^{ +4.7 }_{ -4.8 } & 0.43 & \cite{petigura17}\\
Kepler-101 b & 2 & 5.77^{ +0.85 }_{ -0.79 } & 51.1^{ +5.1 }_{ -4.7 } & 1.46^{ +0.90 }_{ -0.50 } & 0.0860^{ +0.0800 }_{ -0.0590 } & 1547 & 81.4^{ +6.8 }_{ -7.5 } & 0.33 & \cite{Bonomo14}\\
Kepler-87 c & 2 & 6.14^{ +0.29 }_{ -0.29 } & 6.4^{ +0.8 }_{ -0.8 } & 0.15^{ +0.03 }_{ -0.03 } & 0.0390^{ +0.0120 }_{ -0.0120 } & 440 & 69.3^{ +2.6 }_{ -3.6 } & -0.17 & \cite{Ofir14}\\
HATS-7 b & 1 & 6.31^{ +0.52 }_{ -0.38 } & 38.1^{ +3.8 }_{ -3.8 } & 0.83^{ +0.23 }_{ -0.17 } & \nodata  & 1070 & 69.6^{ +4.9 }_{ -6.7 } & 0.25 & \cite{Bakos15}. NEA gives no age estimate. Adopted $5\pm2Gyr$\\
HAT-P-26 b & 1 & 6.33^{ +0.81 }_{ -0.36 } & 18.8^{ +2.2 }_{ -2.2 } & 0.40^{ +0.15 }_{ -0.10 } & 0.1240^{ +0.0600 }_{ -0.0600 } & 981 & 67.8^{ +6.1 }_{ -7.2 } & -0.04 & \cite{Hartman11}\\
CoRoT-8 b & 1 & 6.39^{ +0.22 }_{ -0.22 } & 69.9^{ +9.5 }_{ -9.5 } & 1.47^{ +0.27 }_{ -0.25 } & \nodata  & 844 & 70.1^{ +2.4 }_{ -3.4 } & 0.30 & \cite{Borde10}. NEA gives age of 3 Gyr. With no uncertanties. Adopted $3\pm1Gyr$\\
Kepler-56 b & 3 & 6.51^{ +0.29 }_{ -0.28 } & 22.1^{ +3.9 }_{ -3.6 } & 0.44^{ +0.10 }_{ -0.09 } & \nodata  & 1479 & 75.7^{ +2.7 }_{ -2.4 } & 0.37 & \cite{Huber13}\\
Kepler-18 d & 3 & 6.98^{ +0.33 }_{ -0.33 } & 16.4^{ +1.4 }_{ -1.4 } & 0.26^{ +0.05 }_{ -0.04 } & 0.0000^{ + }_{  } & 784 & 59.2^{ +3.3 }_{ -3.6 } & 0.19 & \cite{Cochran11}\\
Kepler-79 d & 4 & 7.16^{ +0.13 }_{ -0.16 } & 6.0^{ +2.1 }_{ -1.6 } & 0.09^{ +0.03 }_{ -0.03 } & 0.0250^{ +0.0590 }_{ -0.0230 } & 626 & 62.6^{ +4.2 }_{ -2.8 } & -0.02 & \cite{Jontof-Hutter14}.\\
K2-24 c & 2 & 7.82^{ +0.72 }_{ -0.72 } & 27.0^{ +6.9 }_{ -6.9 } & 0.31^{ +0.14 }_{ -0.10 } & \nodata  & 605 & 47.7^{ +7.9 }_{ -9.6 } & 0.42 & \cite{Petigura16}\\
KOI-367 b & 1 & 5.03_{ -0.53 }^{+0.53} & 48.5_{ -3.68}^{+3.99} & 2.11_{ -0.56 }^{+0.86} & 0.833_{-0.013}^{+0.013} & 652 & 82.2_{-6.2}^{+5.9} & 0.189 & This work\\

==> tab_subsaturns.tex <==
% pl_name pl_radius pl_mass pl_density pl_orbeccen pl_teq pl_fenv st_metfe
Kepler-4 b & 1 & 4.00^{ +0.21 }_{ -0.21 } & 24.5^{ +3.8 }_{ -3.8 } & 2.09^{ +0.53 }_{ -0.44 } & \nodata  & 1597 & 6.7^{ +1.3 }_{ -1.4 } & +0.17\\
GJ 436 b & 1 & 4.17^{ +0.17 }_{ -0.17 } & 22.1^{ +2.3 }_{ -2.3 } & 1.67^{ +0.30 }_{ -0.26 } & 0.1383^{ +0.0002 }_{ -0.0002 } & 659 & 12.6^{ +1.9 }_{ -1.9 } & \nodata \\
Kepler-11 e & 6 & 4.19^{ +0.07 }_{ -0.09 } & 8.0^{ +1.5 }_{ -2.1 } & 0.60^{ +0.15 }_{ -0.14 } & 0.0120^{ +0.0060 }_{ -0.0060 } & 630 & 14.9^{ +0.7 }_{ -0.7 } & -0.04\\
Kepler-413 b & 1 & 4.35^{ +0.10 }_{ -0.10 } & 51.0^{ +22.0 }_{ -21.0 } & 2.40^{ +1.00 }_{ -1.00 } & 0.1185^{ +0.0018 }_{ -0.0017 } & 348 & 10.8^{ +3.8 }_{ -2.0 } & \nodata \\
K2-27 b & 1 & 4.48^{ +0.23 }_{ -0.23 } & 30.9^{ +4.6 }_{ -4.6 } & 1.88^{ +0.46 }_{ -0.38 } & 0.2510^{ +0.0880 }_{ -0.0880 } & 910 & 13.9^{ +2.4 }_{ -2.5 } & +0.13\\
Kepler-223 e & 4 & 4.60^{ +0.27 }_{ -0.41 } & 4.8^{ +1.4 }_{ -1.2 } & 0.27^{ +0.11 }_{ -0.09 } & 0.0510^{ +0.0190 }_{ -0.0190 } & 944 & 16.5^{ +2.5 }_{ -2.6 } & +0.06\\
HAT-P-11 b & 1 & 4.73^{ +0.16 }_{ -0.16 } & 25.7^{ +2.9 }_{ -2.9 } & 1.34^{ +0.22 }_{ -0.20 } & 0.1980^{ +0.0460 }_{ -0.0460 } & 861 & 17.1^{ +1.5 }_{ -1.5 } & +0.31\\
K2-32 b & 3 & 5.13^{ +0.28 }_{ -0.28 } & 16.5^{ +2.7 }_{ -2.7 } & 0.67^{ +0.18 }_{ -0.15 } & \nodata  & 815 & 22.5^{ +3.0 }_{ -3.1 } & -0.02\\
Kepler-25 c & 3 & 5.20^{ +0.09 }_{ -0.09 } & 24.6^{ +5.7 }_{ -5.7 } & 0.96^{ +0.24 }_{ -0.23 } & \nodata  & 1018 & 21.4^{ +1.3 }_{ -1.3 } & -0.04\\
Kepler-223 d & 4 & 5.24^{ +0.26 }_{ -0.45 } & 8.0^{ +1.5 }_{ -1.3 } & 0.30^{ +0.10 }_{ -0.07 } & 0.0370^{ +0.0180 }_{ -0.0170 } & 1040 & 22.3^{ +3.4 }_{ -3.2 } & +0.06\\
K2-108 b & 1 & 5.28^{ +0.54 }_{ -0.54 } & 59.4^{ +4.4 }_{ -4.4 } & 2.21^{ +0.90 }_{ -0.59 } & 0.1800^{ +0.0420 }_{ -0.0420 } & 1440 & 16.0^{ +4.8 }_{ -5.4 } & +0.33\\
Kepler-18 c & 3 & 5.49^{ +0.26 }_{ -0.26 } & 17.3^{ +1.9 }_{ -1.9 } & 0.57^{ +0.12 }_{ -0.10 } & \nodata  & 979 & 25.7^{ +2.6 }_{ -2.8 } & +0.19\\
K2-24 b & 2 & 5.68^{ +0.56 }_{ -0.56 } & 21.0^{ +5.4 }_{ -5.4 } & 0.62^{ +0.31 }_{ -0.22 } & \nodata  & 766 & 28.4^{ +7.4 }_{ -6.2 } & +0.42\\
K2-39 b & 1 & 5.71^{ +0.63 }_{ -0.63 } & 39.7^{ +4.6 }_{ -4.6 } & 1.16^{ +0.54 }_{ -0.34 } & 0.1500^{ +0.0760 }_{ -0.0760 } & 1689 & 18.1^{ +5.2 }_{ -4.8 } & +0.43\\
Kepler-101 b & 2 & 5.77^{ +0.85 }_{ -0.79 } & 51.1^{ +5.1 }_{ -4.7 } & 1.46^{ +0.90 }_{ -0.50 } & 0.0860^{ +0.0800 }_{ -0.0590 } & 1547 & 19.5^{ +7.9 }_{ -6.9 } & +0.33\\
Kepler-87 c & 2 & 6.14^{ +0.29 }_{ -0.29 } & 6.4^{ +0.8 }_{ -0.8 } & 0.15^{ +0.03 }_{ -0.03 } & 0.0390^{ +0.0120 }_{ -0.0120 } & 440 & 35.6^{ +3.4 }_{ -3.7 } & -0.17\\
HATS-7 b & 1 & 6.31^{ +0.52 }_{ -0.38 } & 38.1^{ +3.8 }_{ -3.8 } & 0.83^{ +0.23 }_{ -0.17 } & \nodata  & 1070 & 33.3^{ +6.1 }_{ -5.8 } & +0.25\\
HAT-P-26 b & 1 & 6.33^{ +0.81 }_{ -0.36 } & 18.8^{ +2.2 }_{ -2.2 } & 0.40^{ +0.15 }_{ -0.10 } & 0.1240^{ +0.0600 }_{ -0.0600 } & 981 & 35.8^{ +6.9 }_{ -7.5 } & -0.04\\
CoRoT-8 b & 1 & 6.39^{ +0.22 }_{ -0.22 } & 69.9^{ +9.5 }_{ -9.5 } & 1.47^{ +0.27 }_{ -0.25 } & \nodata  & 844 & 32.2^{ +3.5 }_{ -3.1 } & +0.30\\
Kepler-56 b & 3 & 6.51^{ +0.29 }_{ -0.28 } & 22.1^{ +3.9 }_{ -3.6 } & 0.44^{ +0.10 }_{ -0.09 } & \nodata  & 1479 & 26.3^{ +2.4 }_{ -2.4 } & +0.37\\
Kepler-18 d & 3 & 6.98^{ +0.33 }_{ -0.33 } & 16.4^{ +1.4 }_{ -1.4 } & 0.26^{ +0.05 }_{ -0.04 } & \nodata  & 784 & 44.5^{ +3.2 }_{ -3.6 } & +0.19\\
Kepler-79 d & 4 & 7.16^{ +0.13 }_{ -0.16 } & 6.0^{ +2.1 }_{ -1.6 } & 0.09^{ +0.03 }_{ -0.03 } & 0.0250^{ +0.0590 }_{ -0.0230 } & 626 & 42.6^{ +2.5 }_{ -3.3 } & -0.02\\
K2-24 c & 2 & 7.82^{ +0.72 }_{ -0.72 } & 27.0^{ +6.9 }_{ -6.9 } & 0.31^{ +0.14 }_{ -0.10 } & \nodata  & 605 & 57.3^{ +9.1 }_{ -9.9 } & +0.42\\
KOI-367 b & 1 & 5.03_{ -0.53 }^{+0.53} & 48.5_{ -3.68}^{+3.99} & 2.11_{ -0.56 }^{+0.86} & 0.833_{-0.013}^{+0.013} & 652 & 82.2_{-6.2}^{+5.9} & +0.189\\
